Contrastive Adapters for Foundation Model Group Robustness

While large pretrained foundation models (FMs) have shown remarkable zero-shot classification robustness to dataset-level distribution shifts, their robustness to subpopulation or group shifts is relatively underexplored. We study this problem, and find that FMs such as CLIP may not be robust to various group shifts. Across 9 robustness benchmarks, zero-shot classification with their embeddings results in gaps of up to 80.7 percentage points (pp) between average and worst-group accuracy. Unfortunately, existing methods to improve robustness require retraining, which can be prohibitively expensive on large foundation models. We also find that efficient ways to improve model inference (e.g., via adapters, lightweight networks with FM embeddings as inputs) do not consistently improve and can sometimes hurt group robustness compared to zero-shot (e.g., increasing the accuracy gap by 50.1 pp on CelebA). We thus develop an adapter training strategy to effectively and efficiently improve FM group robustness. Our motivating observation is that while poor robustness results from groups in the same class being embedded far apart in the foundation model "embedding space," standard adapter training may not bring these points closer together. We thus propose contrastive adapting, which trains adapters with contrastive learning to bring sample embeddings close to both their ground-truth class embeddings and other sample embeddings in the same class. Across the 9 benchmarks, our approach consistently improves group robustness, raising worst-group accuracy by 8.5 to 56.0 pp over zero-shot. Our approach is also efficient, doing so without any FM finetuning and only a fixed set of frozen FM embeddings. On benchmarks such as Waterbirds and CelebA, this leads to worst-group accuracy comparable to state-of-the-art methods that retrain entire models, while only training $\leq$1% of the model parameters.

==> abstract.tex <==
\begin{abstract}
\noindent
While large pretrained foundation models (FMs) have shown remarkable zero-shot classification robustness to dataset-level distribution shifts, their robustness to subpopulation or group shifts is relatively underexplored.
%
We study this problem, and find that foundation models such as CLIP may not be robust to various group shifts. Across 9 robustness benchmarks, zero-shot classification with their embeddings results in gaps of up to 80.7 percentage points (pp) between average and worst-group accuracy. 
%
Unfortunately, existing methods to improve robustness require retraining, which can be prohibitively expensive on large foundation models. We also find that efficient ways to improve model inference (\eg{} via adapters, lightweight networks that transform FM embeddings) do not consistently improve and can sometimes \emph{hurt} group robustness compared to zero-shot (\eg{}  increasing the accuracy gap by 50.1 pp on CelebA). 
%
We therefore develop an adapter training strategy to effectively and efficiently improve FM group robustness. Our motivating observation is that while poor robustness results from groups in the same class being embedded far apart in the foundation model ``embedding space,'' standard adapter training may not bring these points closer together. We thus propose contrastive adapting, which contrastively trains adapters to bring sample embeddings close to both their ground-truth class embeddings \emph{and} \emph{other sample} embeddings in the same class.
% 
Across the 9 benchmarks, contrastive adapting consistently improves group robustness, raising worst-group accuracy by 8.5 to 56.0 pp over zero-shot. Our approach is also efficient, doing so without any FM finetuning and only a fixed set of frozen FM embeddings. On popular benchmarks such as Waterbirds and CelebA, this leads to worst-group accuracy comparable to state-of-the-art methods that retrain entire models, while only training $\leq$1\% of the model parameters.
%
% Finally, we derive supporting theory that suggests the contrastive adapting loss can play a key role upper-bounding the robustness gap in foundation model adapter settings.

% in the foundation model adapter setting.


% In addition, these adapter strategies also outperform comparable approaches that also only require fixed FM embeddings, scale across various foundation model architectures, and enable group robust classification that rivals that of much larger models trained with state-of-the-art robustness techniques, while only using a fraction of their compute resources.   
% and performs similarly to ERM-trained adapters in the group-balanced setting.
% Among methods that only require access to a fixed set of FM embeddings, \name{} also outperforms existing comparable approaches by \fillin{} to \fillin{} pp across both group-balanced and imbalanced data settings, while performing similarly to ERM-trained adapters in the group-balanced setting.
% 
% and with just $1$\% of the trainable parameters, \name{} outperforms ResNet-50 models trained with state-of-the-art robustness methods by \fillin{} and \fillin{} pp on the popular Waterbirds and CelebA robustness benchmarks.
%
% To understand these improvements, we analyze the adapter setting, and find that under Lipschitzness properties of the pretrained FM embeddings, \name{}'s optimization objective can bound the worst-group versus average accuracy gap \temp{(working result)}.
% and global structure given by using pretrained embeddings as inputs to show that \textfillin{}.



\end{abstract}



==> abstract_submit.tex <==
\begin{abstract}
While foundation models (FMs) have shown remarkable zero-shot classification robustness to dataset-level distribution shifts, their robustness to subpopulation or group shifts, is relatively underexplored. We study this problem, and find that foundation models such as CLIP may not be robust to various group shifts. Across 9 robustness benchmarks, zero-shot classification with their embeddings results in gaps of up to 80.7 percentage points (pp) between average and worst-group accuracy. Unfortunately, existing techniques to improve robustness require model retraining, which may make them less accessible with foundation models. Accessible ways to improve foundation model inference (e.g., via adapters) do not consistently improve robustness, and can lead to *poorer* worst-group accuracy than zero-shot. We therefore propose an adapter training strategy to effectively yet accessibly improve foundation model group robustness. Our motivating observation is that while poor robustness results from groups in the same class being embedded far apart in the foundation model embedding space, training adapters with standard empirical risk minimization (ERM) may not actually bring these points closer together. Our approach is thus a simple contrastive adapter training method, which trains adapters to not only output sample embeddings closer to their ground-truth class embeddings, but also encourages learning similar embeddings for samples initially far apart but in the same class. Across the same 9 robustness benchmarks, our approach substantially and consistently improves group robustness, raising worst-group accuracy by 23.4 to 60.0 pp over zero-shot classification. Our approach is also accessible, doing so without *any* finetuning and only requiring a fixed set of foundation model embeddings. On popular robustness datasets, this allows us to achieve near state-of-the-art worst-group accuracy while only training 0.1% of comparable methods' parameters. Finally, we support our approach with theory that suggests optimizing the contrastive loss can play a key role in bounding the worst-group versus average accuracy gap in the foundation model adapter setting.

\end{abstract}



==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\subsection{Notation and setup}
Consider samples $(x, y, g) \sim P$, where $x \in \cX$ are input features, $y \in \cY$ is a class label, and $g$ is an unobserved group label. $P$ is the unknown population distribution. 

Let $G$ be the set of all groups, and $G_y$ be the set of groups with label $y$ in $G$. Let $\cL_\text{wg}$ be the worst-group loss in $\cG_y$

For any label $y \in \mathcal{Y}$, let $G_y$ be the set of groups with label 



==> introduction_5_12.tex <==
\section{Introduction}

Foundation models (FMs)---large pretrained models trained on massive datasets---offer an exciting new paradigm for deep learning. Recent works have shown that without any finetuning, zero-shot classification with foundation model embeddings can accurately generalize to various datasets \cite{brown2020language, radford2021learning, jia2021scaling, singh2021flava}, while also exhibiting impressive robustness to dataset-level distribution shifts \citep{kumar2022fine, wortsman2021robust}. Instead of training task-specific models, practitioners can seemingly now use a single foundation model's pretrained embeddings for accessible and effective inference on a variety of tasks. 

However, despite these narratives of improved generalization and robustness, a critical yet underexplored question is how robust foundation models are to distribution shifts \emph{between} subpopulations or ``groups'' in data. Prior works have established that this group robustness---\ie{} performing well on all groups---is a fundamental challenge for modern deep learning \cite{sagawa2020investigation, sohoni2020no, nam2020learning, beery2018recognition, buolamwini2018gender, oakden2020hidden, koh2021wilds}. Yet most prior FM evaluations focus on overall population-level performance or dataset-level distribution shifts \citep{radford2021learning, kumar2022fine, wortsman2021robust}; they do not evaluate foundation model performance on individual groups.

% perform on individual groups---or meaningful subpopulations---of data. 
% % Despite growing narratives of improved generalization and robustness, 
% Most prior FM evaluations focus on overall population-level performance or dataset-level distribution shifts \citep{radford2021learning, kumar2022fine, wortsman2021robust}. They ignore the important issue of \emph{group robustness}, or how robust foundation models are to distribution shifts between groups or subpopulations \emph{within} a dataset \cite{sagawa2019distributionally, liu2021just}. 
% However, prior works have established group robustness as a fundamental real-world challenge for modern deep learning \cite{sagawa2020investigation, sohoni2020no, nam2020learning, beery2018recognition, buolamwini2018gender, oakden2020hidden, koh2021wilds}, and foundation models may also suffer from these same issues.
% ---and how to improve their robustness if these issues do apply---is 
% that limit the success of real-world ML deployments .
% Under such groups shifts, deep learning classifiers can achieve high average performance yet poor performance on individual groups. This limits deep learning deployability in many real-world settings 

In this work, we thus explore the group robustness of popular foundation models, and aim accessible methods to improve their group robustness.
% and understand the settings and mechanisms under which these robustness methods work.
%
We first motivate our study by showing that pretrained foundation models may not be robust to various group shifts. Using a standard prompting approach for zero-shot classification \cite{radford2021learning}, we evaluate \numberFMs{} foundation models on \numberDatasets{} robustness benchmarks,
% with either spurious correlations \cite{liu2015deep, WelinderEtal2010, koh2021wilds} or fine-grained classes \cite{santurkar2020breeds, parkhi2012cats}, 
and find that zero-shot classification with their pretrained embeddings can result in large gaps of up to \temp{80.7} percentage points (pp) between average and \emph{worst-group} accuracy. 
% Our evaluation consists of benchmarks with spurious correlations  and fine-grained classes , illustrating 

We then aim to improve the group robustness of foundation models in an efficient and scalable manner. While improving group robustness in machine learning is a well-studied topic, doing so with foundation models introduces unique challenges.
% the size and accessibility of FMs introduce unique challenges. 
Existing approaches to improve robustness require retraining one (and often more) models with group-balanced data \citep{shimodaira2000improving, sagawa2020investigation, liu2021just, kirichenko2022last} or some robustness objective \citep{sagawa2019distributionally, Ahmed2021SystematicGW, taghanaki2021robust, nam2020learning, sohoni2020no, creager2021environment, zhang2022correct}.
% , often training separate models \emph{in addition} to the desired robust classifier \citep{nam2020learning, sohoni2020no, creager2021environment, liu2021just, zhang2022correct, kirichenko2022last}. 
However, applying these methods to retrain foundation model may be prohibitively expensive for individual practitioners. Retraining for individual tasks also runs counter to their promise of accessible and effective zero-shot inference. As such zero-shot paradigms become increasingly prevalent---even today developers might only use APIs to access the embeddings or outputs of increasingly large pretrained foundation models \citefillin{}---it becomes increasingly desirable to improve robustness with limited access to the original pretrained models. 

% methods that can improve robustness with just their embeddings. 

We thus investigate strategies for improving foundation model group robustness without finetuning or accessing the original model weights, only assuming a fixed set of pretrained embeddings computed for a desired task. 
%
To guide our study, we first ask if, despite leading to poor zero-shot robustness, the pretrained embeddings encode enough group information to classify groups correctly. In other words, is improving robustness with just these embeddings even possible? To answer this question, we 


try prompting with group information, fitting \emph{linear probes} (linear classifiers), and training \emph{adapters} (two-layer MLPs), training the latter two on group-balanced foundation model embeddings. We find that these approaches can significantly increase robustness, decreasing the worst-group versus average accuracy gap by \fillin{} to \fillin{}. These results suggest that we \emph{can} improve robustness with just the sample embeddings. However, in practice we may not have training data group information, and our available data may be (unknowingly) group-imbalanced. In these group-imbalanced settings, training linear probes and adapters can result in \emph{poorer} group robustness than zero-shot classification, measured by increases in worst-group versus average accuracy gaps by \fillin{} to \fillin{}. 


We ask if we can improve robustness by either (i) changing the ``prompts'', such that an alternate , or (ii) transforming the sample embeddings, such that we can better ``present'' the latent information for the existing prompt embeddings to separate classes more robustly. 

We therefore focus our study to how to train adapters and linear probes robustly, such that we can improve  Inspired by recent robustness methods, 

, such that we can leverage our available training data to improve robustness without exacerbating poor robustness. Inspired by recent methods, we aim to train adapters such that they can leverage

The initial embeddings carry the relevant information 


on \fillin{} out of \fillin{} of the original robustness benchmarks. This suggests that the initial sample embeddings encode the relevant information, the original prompts or the initial sample embeddings were just insufficient for separating by or presenting this information. 

However, all of these approaches rely on having  

Our results suggest that the pretrained embeddings

We first aim to determine if this is even possible. In other words, do the out-of-the-box sample embeddings encode the relevant information to classify groups correctly, but was it just the case that our prompts or the initial sample embeddings were insufficient for separating by or presenting this information? 
%
We answer this question by fitting \emph{linear probes} (linear classifiers), using prompts with additional group information, and training \emph{adapters} (two-layer bottleneck MLPs) on top of pretrained embeddings. These simple approaches can
% simply using group-informed prompts and training these models with empirical risk minimization (ERM) on group-balanced data can 
significantly increase worst-group performance (by \fillin{} to \fillin{}) and decrease the worst-group vs average accuracy gap (by \fillin{} to \fillin{}), suggesting that the pretrained foundation model embeddings are often sufficient for group-robust classification. The relevant information is in the embeddings; we just need to learn how to classify by it.

it the case that either (i) our prompts failed to separate the sample embeddings by this information or (ii) the out-of-the-box sample embeddings failed to ``present'' this information 

were either poor prompts or the 


but t

better ``present'' representations such that the class 

We answer this by training 


In other words, is the class-relevant information latent in the embeddings, but are either the embeddings as is or the prompting a poor way to 

is the information in the embeddings, but was  

Can we separate out this information 
was our prompting just a poor way to separate samples by this information?
% improving group robustness with just these embeddings is even possible. Do the embeddings encode the relevant class information for each group, but was our prompting just a poor way to separate samples by this information?
% and was the poor zero-shot group robustness merely due to suboptimal prompting that fails to separate samples by this information?
% doing so is even possible. Is the poor zero-shot  the pretrained model embeddings retain 
% doing so is even possible. 
% possible to improve robustness with just the embeddings. Do the FM embeddings retain the relevant group information, but is prompting just a poor way to discriminate samples by this information?
% In doing so, we also aim to answer if FM embeddings retain the relevant information required to classify groups; zero-shot classification may just be a poor way to extract this information.
% We focus on training adapters---small lightweight MLPs---that take  pretrained FM sample embeddings as inputs. 
% In the zero-shot paradigm, this has the advantage of keeping costs fixed, as we only need to compute a fixed set of sample and class embeddings once, and only requires updating 0.05\% to 0.25\% of the weights needed to finetune FMs. 
% Because we train on top of the same embeddings that lead to poor zero-shot robustness, we also seek to understand if the poor zero-shot performance is because the pretrained FM embeddings do not have sufficient
We answer this question by training \emph{linear probes} (linear classifiers) and \emph{adapters} (two-layer bottleneck MLPs) on top of pretrained FM sample embeddings from group-balanced data. We find that simply training these models with empirical risk minimization (ERM) can significantly increase worst-group performance (by \fillin{} to \fillin{} pp) and decrease the worst-group versus average performance gap (by \fillin{} to \fillin{} pp). 
% Surprisingly, using just \fillin{} samples per group, we can significantly improve worst-group accuracy by \fillin{} to \fillin{} pp. 
This suggests that pretrained FM embeddings are often sufficient for group-robust classification. The group information is in the embeddings; we just need to learn how to extract and classify by it.  

However, doing so in practice can be non-trivial. We may not always have group labels or metadata for our samples, such that task training data may be (unknowingly) group-imbalanced. With group-imbalanced data, we find that linear probes and adapters trained with ERM can result in \emph{poorer} group robustness than zero-shot classification, measured by drops in worst-group accuracy by \temp{-X} to \temp{-X} pp.
% if we do not have group information and task training samples are imbalanced, we find that training 
%%
% we may not always have group information for the entire available task data. We then ask if 
%%
% As a first step, we consider training adapters---lightweight bottleneck MLPs---on top of pretrained FM sample embeddings with standard empirical risk minimization (ERM). 
% % While using embeddings as inputs allows us to train efficiently and avoid processing complex input modalities, it raises the question of if improving 
% Surprisingly, ERM-trained adapters can significantly improve worst-group accuracy on \temp{\emph{M}} out of \temp{11} group robustness benchmarks, despite the same input embeddings leading to poor worst-group accuracy via zero-shot classification. 
% % Studying this further, 
% We find that a crucial deciding factor for ERM adapter success is whether the worst-group versus average accuracy gap occurs across evenly-sized, balanced groups. 
% % Zero-shot classification can still result in poor robustness in group-balanced settings, 
% In group-balanced settings, ERM adapters improve worst-group and average accuracy by up to \fillin{} to \fillin{} pp respectively.
% % This is in line with prior works, which show that training adapters on class or group-balanced datasets can significantly improve task-specific accuracy \citefillin{}. 
% %
% However, if groups are imbalanced, ERM adapters can result in \emph{poorer} robustness than zero-shot classification, measured by drops in worst-group accuracy by \temp{-X} to \temp{-X} pp. 
% % This also echoes prior work in robustness, where practitioners may also not have sufficient labels to identify all groups, limiting the ability to rebalance these datasets.

To then handle the group-imbalanced setting, we propose \name{}, a contrastive adapter training strategy. The key idea is to train adapters to pull sample embeddings with the same class but different zero-shot FM predictions closer together, while ``pushing apart'' sample embeddings with different ground-truth classes but the same zero-shot predictions. 
%
\name{} improves robustness on the remaining \temp{\emph{K}} out of \temp{11} datasets, raising worst group accuracy by \fillin{} to \fillin{} pp over zero-shot classification without requiring any training group labels. Furthermore, name performs better than comparable methods that also only require FM embeddings by \fillin{} to \fillin{} pp, and outperforms other no-finetuning FM methods such as prompt engineering (with group information) by \fillin{} to \fillin{} pp. Notably, on standard robustness benchmarks such as Waterbirds and CelebA, \name{} adapters outperform much larger ResNet-50s trained with state-of-the-art robustness methods, achieving \fillin{} to \fillin{} pp higher worst-group accuracy while only updating \temp{0.1\%} of the parameters and using \temp{11\%} of the training time. 
%
By extending \name{} with a simple heuristic based on \textfillin{} to determine when to train adapters with ERM or contrastive learning, we improve robustness across all \temp{11} datasets by up to \fillin{} pp.
% propose a simple selection strategy based on \textfillin{} to determine when to use ERM or \name{} adapters, which improves robustness across all \temp{11} datasets by up to \fillin{} pp. 
Our results suggest that FM embeddings often do retain the relevant information to achieve high group robustness, and that adapters are an effective way to extract this information and improve robustness. 

Finally, to understand these gains, we theoretically analyze the adapter setting \temp{[\emph{result}]} \todo{fill in}

% . We show that, using properties of local Lipschitzness preserved by working with pretrained model embeddings as inputs, 

% We draw connections between \fillin{} and \fillin{} to show why training with adapters can improve worst-group accuracy. Notably, because we train with pretrained model embeddings as inputs, we can use local Lipschitzness and global structure assumptions for our data inputs to show that \temp{[\emph{result}]}. We further support our theory with additional empirical ablations, showing that the adapter setting allows us to realistically apply these assumptions to explain the empirical behavior of the adapters.  

% We summarize our contributions as follows:
% \begin{itemize}[leftmargin=*]
%     \item We demonstrate that group robustness is a critical problem for foundation models.
%     \item We show that we can use adapters to substantially improve the group robustness of these models. These results suggest that poor zero-shot robustness is not because FM embeddings do not retain relevant group information, but rather that we need the right methods to extract and apply this information.
%     % despite FM embeddings leading to poor group robustness in zero-shot pipelines, we can use adapters to extract group information and substantially improve group robustness.
%     \item We theoretically analyze the adapter setting, and \temp{[\emph{something summarizing the theory}]}
% \end{itemize}



==> introduction_5_13.tex <==
\section{Introduction}

Foundation models (FMs)---large pretrained models trained on massive datasets---offer an exciting new paradigm for deep learning. Recent works have shown that without any finetuning, zero-shot classification with foundation model embeddings can accurately generalize to various datasets \cite{brown2020language, radford2021learning, jia2021scaling, singh2021flava}, while also exhibiting impressive robustness to dataset-level distribution shifts \citep{kumar2022fine, wortsman2021robust}. Instead of training task-specific models, practitioners can seemingly now use a single foundation model's pretrained embeddings for accessible and effective inference on a variety of tasks. 

However, despite these narratives of improved generalization and robustness, a critical yet underexplored question is how robust foundation models are to distribution shifts \emph{between} subpopulations or ``groups'' in data. Prior works have established that this group robustness---\ie{} performing well on all groups---is a fundamental challenge for modern deep learning \cite{sagawa2020investigation, sohoni2020no, nam2020learning, beery2018recognition, buolamwini2018gender, oakden2020hidden, koh2021wilds}. Yet most prior FM evaluations focus on overall population-level performance or dataset-level distribution shifts \citep{radford2021learning, kumar2022fine, wortsman2021robust}; they do not evaluate foundation model performance on individual groups.

% perform on individual groups---or meaningful subpopulations---of data. 
% % Despite growing narratives of improved generalization and robustness, 
% Most prior FM evaluations focus on overall population-level performance or dataset-level distribution shifts \citep{radford2021learning, kumar2022fine, wortsman2021robust}. They ignore the important issue of \emph{group robustness}, or how robust foundation models are to distribution shifts between groups or subpopulations \emph{within} a dataset \cite{sagawa2019distributionally, liu2021just}. 
% However, prior works have established group robustness as a fundamental real-world challenge for modern deep learning \cite{sagawa2020investigation, sohoni2020no, nam2020learning, beery2018recognition, buolamwini2018gender, oakden2020hidden, koh2021wilds}, and foundation models may also suffer from these same issues.
% ---and how to improve their robustness if these issues do apply---is 
% that limit the success of real-world ML deployments .
% Under such groups shifts, deep learning classifiers can achieve high average performance yet poor performance on individual groups. This limits deep learning deployability in many real-world settings 

In this work, we thus first explore the group robustness of popular foundation models, before primarily investigating accessible methods to improve their group robustness.
% and understand the settings and mechanisms under which these robustness methods work.
%
We first motivate our study by showing that pretrained foundation models may not be robust to various group shifts. Using a standard prompting approach for zero-shot classification \cite{radford2021learning}, we evaluate \numberFMs{} foundation models on \numberDatasets{} robustness benchmarks,
% with either spurious correlations \cite{liu2015deep, WelinderEtal2010, koh2021wilds} or fine-grained classes \cite{santurkar2020breeds, parkhi2012cats}, 
and find that zero-shot classification with their pretrained embeddings can result in large gaps of up to \temp{80.7} percentage points (pp) between average and \emph{worst-group} accuracy. 
% Our evaluation consists of benchmarks with spurious correlations  and fine-grained classes , illustrating 

We then aim to improve the group robustness of foundation models in an efficient and scalable manner. While improving group robustness in machine learning is a well-studied topic, doing so with foundation models introduces unique challenges.
% the size and accessibility of FMs introduce unique challenges. 
Existing approaches to improve robustness require retraining models with group-balanced data \citep{shimodaira2000improving, sagawa2020investigation, liu2021just, kirichenko2022last} or some robustness objective \citep{sagawa2019distributionally, Ahmed2021SystematicGW, taghanaki2021robust, nam2020learning, sohoni2020no, creager2021environment, zhang2022correct}.
% , often training separate models \emph{in addition} to the desired robust classifier \citep{nam2020learning, sohoni2020no, creager2021environment, liu2021just, zhang2022correct, kirichenko2022last}. 
However, applying these methods to retrain foundation models may be prohibitively expensive for individual practitioners. Retraining these models for individual tasks also runs counter to their promise of accessible and effective zero-shot inference. As foundation models get larger and the zero-shot paradigm become increasingly prevalent---even today developers might only interact with foundation models via APIs to get embeddings or model outputs \citefillin{}---it becomes increasingly desirable to improve robustness with limited access to the original pretrained models. 

% methods that can improve robustness with just their embeddings. 

We thus investigate strategies for improving foundation model group robustness without finetuning or accessing the original model weights, only assuming access to a fixed set of pretrained embeddings computed for a desired task. 
%
Throughout our study, we aim to determine if, despite leading to poor zero-shot robustness, the pretrained embeddings encode enough class information to classify groups correctly. 
%
To do so, we explore whether we can improve robustness by either (i) \emph{transforming} the pretrained sample embeddings to better ``present'' the class information, such that existing prompt embeddings can separate samples by classes more robustly, or (ii) using alternative prompt embeddings to better separate the existing sample embeddings by their class-specific features.  
%

As a first step to determine if this is possible,
we carry out (i) by training an \emph{adapter} (a two-layer bottleneck MLP) on top of \emph{group-balanced} foundation model sample embeddings, and (ii) by either fitting a linear probe (a linear classifier) on the same embeddings, or using prompts with group information. 
%
We find that simply training both adapters and linear probes in this setup with empirical risk minimization (ERM) can substantially increase robustness, decreasing the worst-group versus average accuracy gap by \fillin{} to \fillin{} pp. These results suggest that we \emph{can} improve robustness with just the sample embeddings. 
%
However, in practice we may not have training data group information, and our available data may be (unknowingly) group-imbalanced. Unfortunately in these settings, training adapters and linear probes with ERM can result in \emph{poorer} group robustness than zero-shot classification, measured by increases in worst-group versus average accuracy gaps by \fillin{} to \fillin{} pp. 

We then focus on improving foundation model group robustness in practical settings where available training data may be group-imbalanced and we do not have training group information. Inspired by recent group robustness, we adapt several prior robustness methods to training adapters and linear probes. We find that doing so can then improve robustness further. Intuitively, we note that zero-shot classification will not be group robust if samples in the same class embed far from each other in the foundation model embedding space. We posit that training adapters or linear probes trains. Inspired by recent work that uses contrastive a, we thus propose a simple contrastive strategy which not only train 

Motivated by prior robustness work, we adapt several methods to training adapters and linear probes. 


We first demonstrate that this is a problem  we try adapting several prior robustness methods to train adapters and linear probes. 

We hypothesize that while the pretrained embeddings contain relevant group information, they also allow adapters or linear probes to learn biases or spurious correlations when training on group-imbalanced data. We thus borrow from recent robustness literature, and adapt several robust training strategies to train adapters and linear probes in our setting. Inspired by the zero-shot classification paradigm which aims to train adapters to match embeddings, we also propose \name{}, a contrastive adapter training strategy that not only trains adapters to output embeddings that match samples' ground-truth prompt embeddings, but also better match the ground-truth sample embeddings. 

Contrastive adapter strategy that not only encourages the adapter to transform embeddings to better match the pretrained class embeddings, but also exploits the inherent foundation model biases by (i) identifying sample embeddings in the same class but embedded ``far away'' in the pretrained foundation model space, (ii) identifying samples in different classes but close in the pretraiend fM space, and learning a

use the training data . Our central strategy is to allow 

Inspired by recent work in robustness and the zero-shot classification protocol, we propose a simple robust adapter training strategy 

therefore  several robust training strategies, such that

Our central guiding principle is to train adapters to no

contain group-irrelevant information (as evidenced by the poor zero-shot robustness), such that training on group-imbalanced data can cause adapters or linear probes to learn group-biased correlations. We therefore explore various approaches to improve robustness. Inspired by, this, we consider training on group

imbalanced training data can exacerbate the group robustness problem by causing adapters or linear probes to learn

We therefore 


To then handle the group-imbalanced setting, we focus on how to . Our 

Inspired by several advances in , we show that 


to output alternative embeddings that better interface with the pretrained 

sample embeddings such that the existing class embeddings can “separate” them by classes more accurately


or (ii) using different ``prompt'' embeddings that can better separate the out-of-the-box sample embeddings by their class-specific features

Use alternative class embeddings to better separate the existing sample embeddings by their inherent class-specific features.



To guide our study, we first ask if, despite leading to poor zero-shot robustness, the pretrained embeddings encode enough group information to classify groups correctly. In other words, is improving robustness with just these embeddings even possible? To answer this question, we 


try prompting with group information, fitting \emph{linear probes} (linear classifiers), and training \emph{adapters} (two-layer MLPs), training the latter two on group-balanced foundation model embeddings. We find that these approaches can significantly increase robustness, decreasing the worst-group versus average accuracy gap by \fillin{} to \fillin{}. These results suggest that we \emph{can} improve robustness with just the sample embeddings. However, in practice we may not have training data group information, and our available data may be (unknowingly) group-imbalanced. In these group-imbalanced settings, training linear probes and adapters can result in \emph{poorer} group robustness than zero-shot classification, measured by increases in worst-group versus average accuracy gaps by \fillin{} to \fillin{}. 


We ask if we can improve robustness by either (i) changing the ``prompts'', such that an alternate , or (ii) transforming the sample embeddings, such that we can better ``present'' the latent information for the existing prompt embeddings to separate classes more robustly. 

We therefore focus our study to how to train adapters and linear probes robustly, such that we can improve  Inspired by recent robustness methods, 

, such that we can leverage our available training data to improve robustness without exacerbating poor robustness. Inspired by recent methods, we aim to train adapters such that they can leverage

The initial embeddings carry the relevant information 


on \fillin{} out of \fillin{} of the original robustness benchmarks. This suggests that the initial sample embeddings encode the relevant information, the original prompts or the initial sample embeddings were just insufficient for separating by or presenting this information. 

However, all of these approaches rely on having  

Our results suggest that the pretrained embeddings

We first aim to determine if this is even possible. In other words, do the out-of-the-box sample embeddings encode the relevant information to classify groups correctly, but was it just the case that our prompts or the initial sample embeddings were insufficient for separating by or presenting this information? 
%
We answer this question by fitting \emph{linear probes} (linear classifiers), using prompts with additional group information, and training \emph{adapters} (two-layer bottleneck MLPs) on top of pretrained embeddings. These simple approaches can
% simply using group-informed prompts and training these models with empirical risk minimization (ERM) on group-balanced data can 
significantly increase worst-group performance (by \fillin{} to \fillin{}) and decrease the worst-group vs average accuracy gap (by \fillin{} to \fillin{}), suggesting that the pretrained foundation model embeddings are often sufficient for group-robust classification. The relevant information is in the embeddings; we just need to learn how to classify by it.

it the case that either (i) our prompts failed to separate the sample embeddings by this information or (ii) the out-of-the-box sample embeddings failed to ``present'' this information 

were either poor prompts or the 


but t

better ``present'' representations such that the class 

We answer this by training 


In other words, is the class-relevant information latent in the embeddings, but are either the embeddings as is or the prompting a poor way to 

is the information in the embeddings, but was  

Can we separate out this information 
was our prompting just a poor way to separate samples by this information?
% improving group robustness with just these embeddings is even possible. Do the embeddings encode the relevant class information for each group, but was our prompting just a poor way to separate samples by this information?
% and was the poor zero-shot group robustness merely due to suboptimal prompting that fails to separate samples by this information?
% doing so is even possible. Is the poor zero-shot  the pretrained model embeddings retain 
% doing so is even possible. 
% possible to improve robustness with just the embeddings. Do the FM embeddings retain the relevant group information, but is prompting just a poor way to discriminate samples by this information?
% In doing so, we also aim to answer if FM embeddings retain the relevant information required to classify groups; zero-shot classification may just be a poor way to extract this information.
% We focus on training adapters---small lightweight MLPs---that take  pretrained FM sample embeddings as inputs. 
% In the zero-shot paradigm, this has the advantage of keeping costs fixed, as we only need to compute a fixed set of sample and class embeddings once, and only requires updating 0.05\% to 0.25\% of the weights needed to finetune FMs. 
% Because we train on top of the same embeddings that lead to poor zero-shot robustness, we also seek to understand if the poor zero-shot performance is because the pretrained FM embeddings do not have sufficient
We answer this question by training \emph{linear probes} (linear classifiers) and \emph{adapters} (two-layer bottleneck MLPs) on top of pretrained FM sample embeddings from group-balanced data. We find that simply training these models with empirical risk minimization (ERM) can significantly increase worst-group performance (by \fillin{} to \fillin{} pp) and decrease the worst-group versus average performance gap (by \fillin{} to \fillin{} pp). 
% Surprisingly, using just \fillin{} samples per group, we can significantly improve worst-group accuracy by \fillin{} to \fillin{} pp. 
This suggests that pretrained FM embeddings are often sufficient for group-robust classification. The group information is in the embeddings; we just need to learn how to extract and classify by it.  

However, doing so in practice can be non-trivial. We may not always have group labels or metadata for our samples, such that task training data may be (unknowingly) group-imbalanced. With group-imbalanced data, we find that linear probes and adapters trained with ERM can result in \emph{poorer} group robustness than zero-shot classification, measured by drops in worst-group accuracy by \temp{-X} to \temp{-X} pp.
% if we do not have group information and task training samples are imbalanced, we find that training 
%%
% we may not always have group information for the entire available task data. We then ask if 
%%
% As a first step, we consider training adapters---lightweight bottleneck MLPs---on top of pretrained FM sample embeddings with standard empirical risk minimization (ERM). 
% % While using embeddings as inputs allows us to train efficiently and avoid processing complex input modalities, it raises the question of if improving 
% Surprisingly, ERM-trained adapters can significantly improve worst-group accuracy on \temp{\emph{M}} out of \temp{11} group robustness benchmarks, despite the same input embeddings leading to poor worst-group accuracy via zero-shot classification. 
% % Studying this further, 
% We find that a crucial deciding factor for ERM adapter success is whether the worst-group versus average accuracy gap occurs across evenly-sized, balanced groups. 
% % Zero-shot classification can still result in poor robustness in group-balanced settings, 
% In group-balanced settings, ERM adapters improve worst-group and average accuracy by up to \fillin{} to \fillin{} pp respectively.
% % This is in line with prior works, which show that training adapters on class or group-balanced datasets can significantly improve task-specific accuracy \citefillin{}. 
% %
% However, if groups are imbalanced, ERM adapters can result in \emph{poorer} robustness than zero-shot classification, measured by drops in worst-group accuracy by \temp{-X} to \temp{-X} pp. 
% % This also echoes prior work in robustness, where practitioners may also not have sufficient labels to identify all groups, limiting the ability to rebalance these datasets.

To then handle the group-imbalanced setting, we propose \name{}, a contrastive adapter training strategy. The key idea is to train adapters to pull sample embeddings with the same class but different zero-shot FM predictions closer together, while ``pushing apart'' sample embeddings with different ground-truth classes but the same zero-shot predictions. 
%
\name{} improves robustness on the remaining \temp{\emph{K}} out of \temp{11} datasets, raising worst group accuracy by \fillin{} to \fillin{} pp over zero-shot classification without requiring any training group labels. Furthermore, name performs better than comparable methods that also only require FM embeddings by \fillin{} to \fillin{} pp, and outperforms other no-finetuning FM methods such as prompt engineering (with group information) by \fillin{} to \fillin{} pp. Notably, on standard robustness benchmarks such as Waterbirds and CelebA, \name{} adapters outperform much larger ResNet-50s trained with state-of-the-art robustness methods, achieving \fillin{} to \fillin{} pp higher worst-group accuracy while only updating \temp{0.1\%} of the parameters and using \temp{11\%} of the training time. 
%
By extending \name{} with a simple heuristic based on \textfillin{} to determine when to train adapters with ERM or contrastive learning, we improve robustness across all \temp{11} datasets by up to \fillin{} pp.
% propose a simple selection strategy based on \textfillin{} to determine when to use ERM or \name{} adapters, which improves robustness across all \temp{11} datasets by up to \fillin{} pp. 
Our results suggest that FM embeddings often do retain the relevant information to achieve high group robustness, and that adapters are an effective way to extract this information and improve robustness. 

Finally, to understand these gains, we theoretically analyze the adapter setting \temp{[\emph{result}]} \todo{fill in}

% . We show that, using properties of local Lipschitzness preserved by working with pretrained model embeddings as inputs, 

% We draw connections between \fillin{} and \fillin{} to show why training with adapters can improve worst-group accuracy. Notably, because we train with pretrained model embeddings as inputs, we can use local Lipschitzness and global structure assumptions for our data inputs to show that \temp{[\emph{result}]}. We further support our theory with additional empirical ablations, showing that the adapter setting allows us to realistically apply these assumptions to explain the empirical behavior of the adapters.  

% We summarize our contributions as follows:
% \begin{itemize}[leftmargin=*]
%     \item We demonstrate that group robustness is a critical problem for foundation models.
%     \item We show that we can use adapters to substantially improve the group robustness of these models. These results suggest that poor zero-shot robustness is not because FM embeddings do not retain relevant group information, but rather that we need the right methods to extract and apply this information.
%     % despite FM embeddings leading to poor group robustness in zero-shot pipelines, we can use adapters to extract group information and substantially improve group robustness.
%     \item We theoretically analyze the adapter setting, and \temp{[\emph{something summarizing the theory}]}
% \end{itemize}



==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:background}
% In this section, we go over the zero-shot classification paradigm with foundation models and review the group robustness problem setting. In each subsection we define relevant notation.
We first describe the group robustness problem setting. We then describe the zero-shot classification protocol made popular with recent vision-language foundation models. In Section~\ref{sec:problem}, we use this protocol to evaluate the zero-shot robustness of various foundation models. In Section~\ref{}, we describe how we train adapters on top of pretrained sample embeddings by building on this protocol.
% We also perform classification with adapters using the core components here.

 

% go over details related to the zero-shot classification paradigm with foundation models and the group robustness problem setting. 
% %
% In each subsection we define relevant notation.

\header{Group robustness} We emphasize robustness to distribution shifts between groups in this work. For setup, we follow prior works \cite{sagawa2019distributionally, sohoni2020no, liu2021just, koh2021wilds} that alternatively describe the phenomenon as \emph{hidden stratification} \cite{sohoni2020no} or \emph{subpopulation shift} \cite{koh2021wilds}. For some task, we have $N$ samples $\{(x_i, y_i, g_i)\}_{i=1}^N$, with sample features or inputs $x_i \in \cX$, class labels $y_i \in \cY$, and group labels $g_i \in \cG$. We use $g_i$ to indicate the group that each sample belongs in, but as in prior work we do not observe group labels during training. Distribution shifts may occur between samples in different groups but the same class. 
% Let $C = |\mathcal{Y}|$ be the number of classes.

Every sample $(x_i, y_i, g_i)$ is drawn from some unknown joint distribution $P$. Let $P_g$ be the specific distribution conditioned on $g$ for any $g \in \mathcal{G}$. For classification loss $\ell : \mathcal{Y} \times \mathcal{Y} \mapsto \mathbb{R}$ and classifier $f_\theta: \mathcal{X} \mapsto \mathcal{Y}$, we want $f_\theta$ to be
accurate, \ie{} achieving low average error:
\begin{equation}
% Keep in mind \exarg{}{}
    \mathcal{L}_\text{avg}(f_\theta) \define \mathbb{E}_{(x, y, g) \sim P} [\ell(f_\theta(x), y)]
\label{eq:average_loss}
\end{equation}
and \emph{group robust}, \ie{}, achieving a small gap between its average error and its worst-group error:
\begin{equation}
% Keep in mind \exarg{}{}
    \mathcal{L}_\text{wg}(f_\theta) \define \max_{g \in \cG}\; \mathbb{E}_{(x, y, g) \sim P_g} [\ell(f_\theta(x), y)]
\label{eq:worst_group_loss}
\end{equation}
Different from domain generalization or out-of-distribution (OOD) evaluation, we observe each group in training, validation, and test splits. However, standard training via empirical risk minimization (ERM) can still lead to poor test set group robustness because training groups may be imbalanced \cite{sagawa2019distributionally, sohoni2020no, zhang2022correct}. 
% the groups may be imbalanced, which can result in poor test set group robustness after standard training via empirical risk minimization (ERM) \cite{sagawa2019distributionally, sohoni2020no, zhang2022correct}. 
% Prior work shows that standard training via empirical risk minimization (ERM) on group-imbalanced training data can result in poor group robustness, \eg{} by learning spurious correlations that hold for larger groups but not smaller ones \cite{sagawa2019distributionally, sohoni2020no, zhang2022correct}. 
% where each group is observed at least once in the training data. However, the groups may be unevenly sized or imbalanced in each data split. Prior work shows that standard training via empirical risk minimization (ERM) can thus resul
% that poor group robustness  
% Prior work primarily shows that poor group robustness---or a large gap between worst-group and average test error---results from imbalanced groups in the training data. Standard training via empirical risk minimization (ERM) can thus result in models learning correlations that hold for the larger groups, but not the smaller ones . 
Here, foundation models are \emph{not trained} on the training data, but we show that zero-shot classification with foundation models can still carry poor group robustness. 

% One possible explanation is that FMs may learn input-target correlations during pretraining that only hold for some but not all downstream data groups \cite{radford2021learning}. We thus aim to improve the group robustness of foundation models

% We thus aim to improve the group robustness of foundation model inference over 

% \citet{radford2021learning} caution that zero-shot models may learn input-target correlations in pretraining data that only hold for some but not all downstream data groups. We would like to improve group robustness 

% In Section~\ref{sec:problem}, we show that this indeed

% When this happens, to improve robustness in an accessible manner, we aim to 

% \eg{} because the models learned correlations in their pretraining data that only hold for some, but not all, groups. 

% \header{Zero-shot robustness of foundation models} Prior works have studied the robustness of foundation model inference and zero-shot classification. \citet{radford2021learning} show that zero-shot CLIP models can be more robust to out-of-distribution shifts than prior ImageNet-trained models, measured via better generalization to various dataset-level distribution shifts on ImageNet classes.
% % to various dataset-level distribution shifts. dataset-level distribution shift
% % measured across various ImageNet-like datasets. 
% % they show that the CLIP models and pretraining data generalize better to various dataset-level distribution shifts
% % dataset-level distribution shifts than prior ImageNet-trained models. 
% However, finetuning CLIP models on downstream data can reduce this robustness. \citet{kumar2022fine, wortsman2021robust} thus propose finetuning methods that improve downstream in-distribution accuracy while maintaining out-of-distribution robustness. Unlike these works, we focus on foundation model robustness to group shifts that occur within a dataset. 
% % We study how well FMs perform on individual data groups, even if we only have class-level prompts. 
% This necessitates evaluating how well FMs perform on individual data groups, as opposed to overall metrics such as average accuracy. We also aim to improve robustness without any foundation model finetuning. 
% \todo{Add discussion on \citet{singla2022core}, which studies how various models (including CLIP models) may rely on spurious artifacts to classify ImageNet images. Add discussion on \citet{berg2022prompt}, which aims to debias CLIP image embeddings using extra metadata (textual concepts or attributes) that the embeddings should ignore.}

% \header{Improving foundation model inference without finetuning} Our work is also related to methods that aim to efficiently improve foundation model downstream performance, without having to finetune or update the original model weights. \emph{Prompt tuning} optimizes the inputs of a FM while keeping the original model weights frozen. Prior works show that optimizing either text \cite{li2021prefix, zhou2021learning, zhou2022conditional, levine2022standing} or image \cite{bahng2022visual, yao2021cpt} inputs can improve a frozen FM's downstream task accuracy. Another line of work adds a small set of parameters to the original FM architecture that are exclusively updated during training. These include low-rank weight matrices \cite{hu2021lora}, linear probes for classification \cite{radford2021learning}, and adapters, small bottleneck MLP layers traditionally interspersed throughout a model \cite{pmlr-v97-houlsby19a, Rebuffi17, pfeiffer-etal-2021-adapterfusion, pfeiffer-etal-2020-adapterhub}. Recently, \citet{gao2021clip} show that a single adapter can be applied on top of CLIP embeddings to improve average downstream task accuracy in a few-shot setting. We instead evaluate how this single adapter paradigm performs in the group robustness setting. We also show that the standard training used by \citet{gao2021clip} can hurt group robustness, and propose alternative training strategies to improve robustness.



\header{Zero-shot classification with foundation models} We review the zero-shot classification paradigm used by recent foundation models \cite{radford2021learning, jia2021scaling, singh2021flava}. 
Consider the data setup above. Let $C = |\mathcal{Y}|$ be the number of all classes. To perform both image and text classification, given a dataset $\{x_n, y_n, g_n\}_{n=1}^N$, we first use a pretrained foundation model to compute $N$ sample and $C$ class embeddings. We then classify each sample by picking the nearest class embedding to its sample embedding. 

% We get sample embeddings by feeding input features $x_n \in \cX$ into an input encoder $f_x :\mathcal{X} \mapsto \cZ$, where $\cZ$ is the pretrained embedding space. For image classification, we treat $\cX$ as image space, and $f_x$ is the image encoder of a vision-language foundation model (\eg{} CLIP). For text classification, we treat $\cX$ as text space, and $f_x$ is the text encoder of a language foundation model (\eg{} GPT-3).

% We get class embeddings by first converting each unique class label $y_c \in \cY$ into a natural language ``prompt'' \eg{} ``a photo of a \texttt{[class name]}'', which lies in text space $\cT$. We then feed each class prompt into the same foundation model's text encoder $f_y : \cT \mapsto \cZ$ to compute our class embeddings. We use $f_x$ and $f_y$ to distinguish the encoder that process sample and class embeddings. However, for text classification this encoder may be the same model. 

% For image classification, $f_X$ and $f_Y$ are different encoders, whereas they may be the same 



% We generalize this framework to both image and text classificatio

For image classification, we get sample embeddings $u_n \in \cZ$ by feeding input image features $x_n \in \mathcal{I}$ into the image encoder $f_I : \mathcal{I} \mapsto \cZ$ of a vision-language foundation model (\eg{} CLIP), where $\cZ$ is the pretrained embedding space. We get class embeddings $v_c \in \cZ$ by first converting each unique class label $y_c \in \cY$ into a natural language ``prompt'' \eg{} ``a photo of a \texttt{[class name]}'', which lies in text space $\cT$. We then feed each class prompt into the vision-language model's text encoder $f_T : \cT \mapsto \cZ$ to compute our class embeddings. 

For text classification, we get both sample and class embeddings with the same text encoder of a language foundation model (\eg{} GPT-3). We compute sample embeddings using the sample text features as inputs $x_n \in \mathcal{T}$, and come up with a prompt for each class as above. 

To perform zero-shot classification for each sample input $\{x_n\}_{n=1}^N$, we use cosine similarity to determine the nearest class embeddings to its sample embedding. 
% for each sample embedding we pick the nearest class embedding via cosine similarity. 
With a temperature parameter $\tau$, we thus classify each sample $x_n$ by whichever class has the highest probability $p^*_n$, where 
\begin{equation}
    p_n^* = \underset{i \in [C]}{\arg \max} \left\{ \frac{\exp(\cos(u_n, v_i) / \tau)}{\sum_{c \in [C]} \exp(\cos(u_n, v_c) / \tau)} \right\}_{i = 1}^C
    \label{eq:zero_shot_classification}
\end{equation}

% we compute the cosine similarity of each sample embedding $u_n$ with every class embedding $\{v_c\}_{c = 1}^C$. With temperature $\tau$, we classify sample $x_n$ by whichever class has the highest probability $p_i^*$, where:
% \begin{equation}
% \hat{y}_n = \arg \max_{c} \big\{\textit{softmax}(\cos(z^x_n, z^y_c) / \tau)) \big\}_{c =1}^C
% \label{eq:zero_shot_classification}
% \end{equation}
% \begin{equation}
%     % p_i = \textit{softmax}(\cos(z^x_n, z^y_c) / \tau))
% p_n^* = \underset{i \in [C]}{\arg \max} \left\{ \frac{\exp(\cos(z^x_n, z^y_i) / \tau)}{\sum_{c \in [C]} \exp(\cos(z^x_n, z^y_c) / \tau)} \right\}_{i = 1}^C
% \label{eq:zero_shot_classification}
% \end{equation}
% \begin{equation}
%     % p_i = \textit{softmax}(\cos(z^x_n, z^y_c) / \tau))
% p_n^* = \underset{i \in [C]}{\arg \max} \left\{ \frac{\exp(\cos(u_n, v_i) / \tau)}{\sum_{c \in [C]} \exp(\cos(u_n, v_c) / \tau)} \right\}_{i = 1}^C
% \label{eq:zero_shot_classification}
% \end{equation}
% \begin{equation}
%     % p_i = \textit{softmax}(\cos(z^x_n, z^y_c) / \tau))
% p_n^* = \underset{i \in [C]}{\arg \max} \Big\{ \frac{\exp(\cos(z^x_n, z^y_i) / \tau)}{\sum_{c \in [C]} \exp(\cos(z^x_n, z^y_c) / \tau)} \Big\}_{i = 1}^C
% \label{eq:zero_shot_classification}
% \end{equation}


% \[
% \hat{y}_n = \arg \max_{c} \frac{\exp\big(\cos(z^x_n, z^Y_c)\big)}{\sum_{c = 1}^C \exp\big(\cos(z^X_n, z^Y_c)\big)}
% \]

% input text features  using the same encoder of a text foundation model (\eg{} GPT-3). 


% To classify samples

% compute class embeddings $z^y_c \in \cZ$ by feeding each prompt, into 

% We then pass this into a text encoder $f_T : \cY$

% we extract sample embeddings $z^x_i \in \cZ$ from input image features $x_i \in \cX$ by using a vision-language foundation model's image enc

% use a vision-language foundation model

% with image encoder  to , where $\cZ$ is the foundation model embedding space. We use the foundation model's text encoder $f_T : \mathcal{T} \mapsto \cZ$ to extract class embeddings $z^y_i \in \cZ$. 

% , and text encoder $f_T : \mathcal{T} \mapsto \cZ$, where $\cZ$ is a shared embedding space. 

% We then classify each sample as the class of the closest class embedding to its sample embedding to the closest class embedding via cosine similarity. More specifically, for image classification we use vision-language FMs with an image encoder $f_X : \mathcal{X} \mapsto \mathcal{Z}$ and a text encoder $f_T : \mathcal{T} \mapsto \mathcal{Z}$ (\eg{} CLIP \cite{radford2021learning} or ALIGN \cite{jia2021scaling}). We first convert each class to a natural language prompt with a template (\eg{} ``This is a \texttt{[class name]}.''), tokenize the prompts to tokens $\{T_c\}_{c=1}^C, T \in  \mathcal{T}$, and obtain class embeddings $f_T(T_c) = z^y_c \in \mathcal{Z}$. We then classify each sample by encoding input $f_X(x_i) = z^x_i \in \mathcal{Z}$ and predicting class $y_i^* = \arg \max_{c} \{\cos (z^x_i, z^y_c)\}_{c = 1}^C$.

% % computing a temperature $\tau$-scaled softmax for each class:
% % \begin{equation}
% % p_{i}^{y} = \frac{\exp( \cos (z^x_i, z^y_i) / \tau)}{\sum_{c = 1}^{C} \exp( \cos (z^x_i, z^y_c) / \tau)}
% % \label{eq:zeroshot_softmax}
% % \end{equation}
% % assigning the highest probability class $y_i$ as the classification. 
% For text classification, we use a text foundation model (\eg{} GPT-3 \cite{brown2020language}) and use the same tokenizer and encoder to process both sample inputs and classes.
% Notably, zero-shot classification only requires a fixed set of $N$ sample embeddings plus $C$ class embeddings, and can perform competitively with more expensive approaches that require \emph{accessing} and \emph{finetuning} entire pretrained models \cite{radford2021learning, jia2021scaling}. Foundation models may thus present a more accessible paradigm for applying powerful deep learning models. If embeddings are all one needs, then while only certain actors may be able to pretrain foundation models, many practitioners can use their outsourced embeddings for relatively low-cost yet effective inference in a variety of downstream applications.

% % However, a core issue limiting this vision is that zero-shot classification with these embeddings may not be perfect for the downstream task. Adding to prior work \citefillin{}, we focus on how to improve the \emph{group robustness} of foundation models while maintaining their promise of wide and accessible downstream transfer, \ie{}, by only assuming access to task-specified pretrained embeddings. 

% % we show that using these embeddings off-the-shelf can critically be not robust to distribution shifts between groups in downstream task data. As a step towards improving the robustness of foundation models while maintaining their promise of wide and accessible downstream transfer, we aim to improve the group robustness of a foundation model while only assuming access to its task-specified embeddings.


% % We finally 

% % discuss the empirical evidence

% % show that zero-shot classification with foundation models can critically not be robust to group shifts, measured via large gaps between worst-group and average accuracy. We finally show that one potential solution, training adapters with available training data via ERM, can significantly improve robustness on some datasets but not others. 

% % and describe our evaluation benchmarks.

% % reporting average and worst-group accuracy across va

% % measure average and worst-gr first describe our experimental setup and give a brief overview of 

% % We use the zero-shot classification across and consider several datasets, divided into those with spurious correlations and those with fine-grained classificatio, dma


==> problem1_zeroshot_robustness.tex <==
% \vspace{-0.25cm}
\section{Problem: zero-shot group-robustness of foundation models}
% \vspace{-0.125cm}
\label{sec:problem}
We present our motivating problem---that zero-shot foundation models may not be robust to various group shifts.  We first describe our experimental setup and benchmarks for evaluating robustness. We then show that FM zero-shot classification can exhibit poor group robustness across these benchmarks, shown via significant gaps between worst-group and average accuracy 

\header{Experimental setup} We evaluate 13 FMs---9 vision-language models (architectures of CLIP \cite{radford2021learning}, CLOOB \cite{furst2021cloob}, and SLIP \cite{mu2021slip}), and 4 large language models (LLM) (architectures of GPT-Neo \citefillin{}, GPT-3 \cite{brown2020language})---across 7 image and 2 text classification datasets respectively. We use zero-shot classification as described in Section~\ref{sec:background}. As recommended by \citet{radford2021learning}, for each dataset we consider several prompt templates. We engineer prompts by using the single best template based on validation worst-group accuracy. In Appendix~\ref{appendix:prompt_list} we list the templates used for each task. 
% We also include additional details on For more details on datasets,
% pretraining models, and experiment protocols,
To benchmark zero-shot group robustness, we use a diverse set of datasets with groups shifts from prior robustness literature. We briefly describe each below, and include additional details in Appendix~\ref{appendix:prompt_list}.
% . We briefly describe each below:
\vspace{-0.125cm}
\begin{itemize}[leftmargin=*]
    \item \textbf{Waterbirds}~\cite{WelinderEtal2010, sagawa2019distributionally}. We classify images by bird type. Each class $\in \{ \texttt{waterbird}, \texttt{landbird} \}$ carries two groups: birds on water backgrounds, and birds on land backgrounds.
    \item \textbf{CelebA}~\cite{liu2015deep, sagawa2019distributionally}. We classify images by celebrity hair color. Each class $\in \{ \texttt{not blond}, \texttt{blond}\}$ carries two groups: celebrities labeled as male, and celebrities labeled as female.
    \item \textbf{BREEDS\myDataset (\texttt{Living-17}, \texttt{Nonliving-26})} ~\cite{santurkar2020breeds}. For the \texttt{Living-17} and \texttt{Nonliving-26} datasets in the BREEDS benchmark sourced from ImageNet~\cite{santurkar2020breeds}, we classify images by one of several categories. Each class is a coarse category consisting of multiple fine-grained groups. Groups in the same class may be visually distinct (\eg{} the \texttt{ape} class includes images of gibbons and gorillas).
    % , and we evaluate over all groups in the original benchmark. 
    % While the original benchmark evaluates how classifiers trained on seen \texttt{source} groups generalize to unseen \texttt{target} groups, we adapt the datasets for our setting by adding 5\% of the images in each \texttt{target} group to the \texttt{source} groups, and evaluating worst-group accuracy over all \texttt{source} and \texttt{target} groups.
    \item \textbf{CIFAR-10.001}, \textbf{CIFAR-10.02} \cite{Krizhevsky2009LearningML, recht2018cifar, lu2020harder}. We classify images by one of 10 categories. We combine CIFAR-10~\cite{Krizhevsky2009LearningML} and either CIFAR-10.1~\cite{recht2018cifar} or CIFAR-10.2~\cite{lu2020harder}, which are collected from different sources. The new datasets' classes carry two groups determined by the source dataset.
    \item \textbf{FMoW-WILDS\myDataset}~\cite{christie2018functional, koh2021wilds}. We classify satellite images into one of 62 building or land-use categories (\eg{} \texttt{airport}, \texttt{zoo}). Each images belongs to one of five groups based on continental region. 
    % We compare the accuracies over all samples in each group as in the WILDS benchmark \cite{koh2021wilds}. 
    % We also evaluate only over test images from the same time period as training images (the ``IID'' split in the original WILDS benchmark \cite{koh2021wilds}). 
    % \item \textbf{iWildCam-WILDS\myDataset}~\cite{beery2021iwildcam, koh2021wilds}. We classify camera trap images by one of 182 animal species. Each class species is divided into groups based on the camera trap deployment. 
    % \item \textbf{MultiNLI}~\cite{williams-etal-2018-broad, sagawa2019distributionally}. We classify whether two text passages entail, are neutral, or contradict each other. Each class carries two groups based on if negation words are present, \eg{} ``no'', ``never''.
    \item \textbf{CivilComments-WILDS}~\cite{DBLP:journals/corr/abs-1903-04561, koh2021wilds}. We classify if a text comment is toxic or not. Samples are organized into 8 groups based on mention of a demographic identity (\eg{} ``female'', ``LGBTQ'').

    \item \textbf{Amazon-WILDS\myDataset}~\cite{ni-etal-2019-justifying, koh2021wilds}. We classify if an online text review is positive or negative. Reviews are organized into different groups based on the product category (\eg{} \texttt{books}, \texttt{electronics}). 
    
\end{itemize}

\header{Zero-shot classification results} Figure~\ref{fig:zeroshot_poor_robustness} shows the worst-group and average accuracies achieved by zero-shot foundation models on various datasets. On all datasets and models, we observe gaps between worst-group versus average accuracy (from 2.7 to 80.7 pp), suggesting that zero-shot classification with FMs may not be robust to group shifts. To rule out poor performance due to sub-optimal prompting, in Appendix~\ref{} we also evaluate clustering the image embeddings for zero-shot classification. This leads to similar results, producing accuracy gaps between \fillin{} and \fillin{} pp.

\begin{figure}
  \centering
  \includegraphics[width=1\textwidth]{figures/zeroshot_barcharts_v0.pdf}
  \vspace{-0.7cm}
  \caption{FM zero-shot classification accuracies. Across datasets and architectures, foundation models can exhibit poor zero-shot group robustness. This is evidenced by gaps of \fillin{} to \fillin{} percentage points (pp) between average (Avg) and worst-group (WG) accuracies.}
  \vspace{-0.25cm}
  \label{fig:zeroshot_poor_robustness}
\end{figure}

% \begin{table}

% {\small
% \centering
% \caption{Vision-language FM zero-shot classification accuracies. Across datasets and architectures, foundation models can exhibit poor zero-shot group robustness. This is evidenced by gaps of \fillin{} to \fillin{} percentage points (pp) between average (Avg) and worst-group (WG) accuracies.}
% \label{table:zero_shot_robustness_results}
% \tabcolsep=0.1cm

% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{@{}ccbcbcbcbcbcbcbcbc@{}}
% \toprule
% \multirow{2}{*}{Model}  & \multirow{2}{*}{Backbone}   & \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA} & \multicolumn{2}{c}{Liv-17} & \multicolumn{2}{c}{NonLiv-26} & \multicolumn{2}{c}{CIFAR-10.001} & \multicolumn{2}{c}{CIFAR-10.02} & \multicolumn{2}{c}{FMoW} & \multicolumn{2}{c}{iWildCam} \\ \cmidrule(l){3-4}\cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12} \cmidrule(l){13-14} \cmidrule(l){15-16} \cmidrule(l){17-18}   
%                         &             & WG             & Avg           & WG           & Avg         & WG           & Avg         & WG            & Avg           & WG              & Avg            & WG             & Avg            & WG          & Avg        & WG            & Avg          \\ \midrule

% % \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{CLIP~\cite{radford2021learning}}}}
% \multirow{5}{*}{CLIP~\cite{radford2021learning}}
% & RN-50   & $36.6$         & $92.2$        & $74.0$       & $81.9$      & $6.0$        & $86.7$      & $6.0$         & $72.8$        & $41.6$          & $70.5$         & $39.1$         & $69.9$         & $10.5$      & $13.2$     & ---           & ---          \\
%                         & RN-101  & $41.8$         & $91.2$        & $46.4$       & $68.5$      & $10.0$       & $88.1$      & $8.0$         & $71.9$        & $60.0$          & $78.1$         & $58.9$         & $77.4$         & $10.5$      & $15.2$     & ---           & ---          \\
%                         & ViT-B/32    & $44.8$         & $87.8$        & $78.4$       & $81.9$      & $16.0$       & $89.0$      & $4.0$         & $74.6$        & $71.9$          & $88.4$         & $68.8$         & $87.3$         & $10.1$      & $16.5$     & ---           & ---          \\
%                         & ViT-B/16    & $25.7$         & $86.2$        & $60.3$       & $75.3$      & $20.0$       & $92.3$      & $4.0$         & $76.9$        & $70.5$          & $89.9$         & $67.5$         & $89.0$         & $14.6$      & $21.5$     & ---           & ---          \\
%                         & ViT-L/14    & $45.0$         & $90.6$        & $71.1$       & $88.1$      & $4.0$        & $94.2$      & $2.0$         & $79.5$        & $86.5$          & $94.9$         & $85.3$         & $94.2$         & $23.0$      & $28.0$     & ---           & ---          \\ \midrule
% % \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{CLOOB~\cite{furst2021cloob}}}}
% \multirow{2}{*}{CLOOB~\cite{furst2021cloob}}  
% & RN-50   & $36.7$         & $61.8$        & $2.7$        & $17.9$      & $4.0$        & $77.9$      & $18.0$        & $43.6$        & $14.4$          & $44.0$         & $18.0$         & $43.6$         & ---         & ---        & ---           & ---          \\
%                         & RN-50x4 & $31.7$         & $75.0$        & --           & --          & $0.0$        & $81.5$      & $7.5$         & $36.0$        & $6.8$           & $36.4$         & $7.5$          & $36.0$         & ---         & ---        & ---           & ---          \\ \midrule
% \multirow{2}{*}{DECLIP~\cite{li2021supervision}} & RN-50   & ---            & ---           & ---          & ---         & ---          & ---         & ---           & ---           & ---             & ---            & ---            & ---            & ---         & ---        & ---           & ---          \\
%                         & ViT-B/32    & ---            & ---           & ---          & ---         & ---          & ---         & ---           & ---           & ---             & ---            & ---            & ---            & ---         & ---        & ---           & ---          \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% }
% \end{table}


% \begin{figure}
% \centering
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{8cm}{0cm}}
% {
%   \caption{Dataset examples illustrating different group shifts and incorrect samples. Table with GPT-Neo, GPT-3, and OPT should be side-by-side to this.}
% }
% \end{figure}

% \begin{table}

% {\small
% \centering
% \caption{Large language model (LLM) zero-shot classification accuracies. LLMs can exhibit poor group robustness, evidenced by gaps of \fillin{} to \fillin{} percentage points (pp) between average and worst-group accuracies.}
% \label{table:zero_shot_robustness_results}
% \tabcolsep=0.1cm

% % \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% LLM                     & Acc. (\%) &  MultiNLI  & CivilComments & Amazon \\ \midrule
% \multirow{2}{*}{GPT-Neo 1.3B}    & Worst-Group        & --     & -- & --        \\
%                           & Average       & --     & -- & --   \\ \midrule
% \multirow{2}{*}{GPT-3 Ada}   & Worst-Group        & --     & -- & --       \\
%                           & Average       & --     & -- & --       \\ \midrule
% \multirow{2}{*}{GPT-3 Babbage} & Worst-Group        & --     & -- & --     \\
%                           & Average       & --     & --& -- &     \\ \midrule
% \multirow{2}{*}{OPT-175B} & Worst-Group        & --    & -- & -- &   \\
%                           & Average       & --     & -- & -- &     \\ \midrule
% \end{tabular}
% % \end{adjustbox}
% }
% \end{table}

% \begin{figure}
% \begin{floatrow}
% \ffigbox{%
%   \rule{3cm}{3cm}%
% }{%
%   \caption{A figure}%
% }
% \capbtabbox{%
%   \begin{tabular}{cc} \hline
%   Author & Title \\ \hline
%   Knuth & The \TeX book \\
%   Lamport & \LaTeX \\ \hline
%   \end{tabular}
% }{%
%   \caption{A table}%
% }
% \end{floatrow}
% \end{figure}

% \header{Implications for improved robustness via embeddings} The results in Table~\ref{table:zero_shot_robustness_results} suggest two hypotheses: (i) the 

% \header{Improving robustness via adapters} To improve robustness, we first consider 



==> problem2_improving_robustness_with_group_info.tex <==
\section{Improving robustness with only foundation model embeddings}
\label{sec:improving_robustness_with_fm_embeddings}
We now aim to improve the robustness of these zero-shot models using only their embeddings. First, in Sec~\ref{sec:do_they_have_the_juice}, we study whether the embeddings carry relevant group group information

\subsection{Do foundation model embeddings encode relevant group information?}
\label{sec:do_they_have_the_juice}

From the results in Table~\ref{table:zero_shot_robustness_results}, we now ask whether it is possible to improve the group robustness of foundation models with just their pretrained embeddings. After all, these embeddings when used in zero-shot classification resulted in poor worst-group accuracy. This raises the possibility that the sample embeddings themselves do not contain the relevant information to classify groups correctly.
% (\temp{temp: \eg{} due to embedding collapse \citefillin{}}). 

To test this hypothesis, we try three strategies to see if sample embeddings encode group information:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Linear probes}: We train a linear classifier $f_\theta : \cZ \mapsto \cY$ which takes pretrained FM sample embeddings as inputs and outputs class predictions. 
    % We use group-balanced data.
    % For sample embedding $x$, class label $y$, we learn weights $\theta := [W, b]$ to minimize the usual cross-entropy loss with predicted probabilities $\hat{y} = Wx + b$
    \item \textbf{Adapters}: We train a single 2-layer MLP $f_\theta : \cZ \mapsto \cZ$ which takes fixed pretrained FM sample embeddings as inputs, passes them through a hidden layer and nonlinearity, and outputs ``updated'' sample embeddings. To classify samples, we use the same zero-shot classification procedure as before, but compute cosine similarities between the new sample embeddings and the fixed pretrained FM class embeddings. 
    % We use group-balanced data.
    \item \textbf{Group-informed prompts}: We update the class embeddings to include group-specific keywords.   by extending the original prompts with group-specific keywords to the original template for each class, inputting these into the foundation model text encoder, and outputting new class embeddings. We then compute cosine similarities between the fixed pretrained FM sample embeddings and the new class embeddings.
\end{enumerate}

Recall that zero-shot classification with FM input and class embeddings is itself a linear classifier, 
% \cite{radford2021learning},
% \[
% \hat{y} = \argmax_{i \in C} \frac{\exp z^y_i z^x}{ \sum_{c \in C} \exp z^y_c z^x}
% \]
where the samples embeddings are the inputs and the class embeddings together make up the weight matrix. The above strategies then reflect alternative ways to update different components of the zero-shot classifier, where the initial weights and sample representations may not interact properly to discriminate samples by group-specific features. 

However, if the original sample embeddings do contain relevant group information, then either updating the zero-shot classifier weights (via linear probes (1)  or group-informed class embeddings (3)) to better discriminate the original sample embeddings with group information in mind, or transforming the sample embeddings (via adapters (2)) to better ``present'' the shared class information across groups, should be able to result in more group-robust classification.

We apply the above to the same group robustness benchmarks in Section~\ref{sec:problem}, training the linear probes and adapters with ERM. For all strategies, we \emph{use group metadata}. As our benchmarks have group-imbalanced training data \cite{sagawa2019distributionally, koh2021wilds}, we rule out the potentially biasing effects of training on such data (reported extensively in prior group robustness work \cite{sagawa2020investigation, liu2021just, nam2020learning, sohoni2020no}) by resampling the training data to have evenly sized groups for each class. The linear probe evaluation is then similar to prior work such as \emph{Deep Feature Reweighting} \cite{kirichenko2022last}, but we do not train the embeddings on the training data first. We defer additional training details to Appendix~\ref{appendix:placeholder}.

In Table~\ref{table:group_balanced_results}, we report results for the CLIP RN-50 and ViT-B/32, DECLIP RN-50 and ViT-B/32, and \textfillin{} models, including the rest in Appendix~\ref{appendix:temp}. Across benchmarks, we observe substantial improvements in worst-group accuracy from \fillin{} to \fillin{} pp, suggesting that foundation model embeddings often do encode information necessary to classify groups correctly. 

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{figures/fig_group_info.pdf}
  \caption{}
  \label{fig:group_balanced_results}
\end{figure*}

\begin{table}[]
\tabcolsep=0.1cm
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
Model                          & Method                        & Acc. (\%) & Waterbirds     & CelebA         & Liv-17         & NonLiv-26      & CIFAR-10.001   & CIFAR-10.02    & FMoW & iWildCam \\ \midrule
\multirow{6}{*}{CLIP RN50}     & \multirow{2}{*}{Linear Probe} & WG        & $76.9 \pm 0.0$ & $77.4 \pm 1.3$ & $46.7 \pm 3.4$ & $29.3 \pm 0.9$ & $16.5 \pm 4.7$ & $55.2 \pm 1.1$ & --   & --       \\
                               &                               & Avg       & $85.3 \pm 0.0$ & $92.0 \pm 0.5$ & $89.3 \pm 0.3$ & $80.3 \pm 0.3$ & $55.5 \pm 0.4$ & $73.1 \pm 0.2$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Adapter}      & WG        & $85.9 \pm 0.0$ & $87.8 \pm 0.5$ & $74.0 \pm 1.6$ & $66.7 \pm 0.9$ & $66.0 \pm 2.0$ & $73.5 \pm 0.5$ & --   & --       \\
                               &                               & Avg       & $87.1 \pm 0.0$ & $92.0 \pm 0.1$ & $94.0 \pm 0.1$ & $91.5 \pm 0.1$ & $80.5 \pm 0.3$ & $83.8 \pm 0.3$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Group Prompt} & WG        & --             & --             & --             & --             & --             & --             & --   & --       \\
                               &                               & Avg       & --             & --             & --             & --             & --             & --             & --   & --       \\ \midrule
\multirow{6}{*}{CLIP RN101}    & \multirow{2}{*}{Linear Probe} & WG        & $77.4 \pm 0.2$ & $84.4 \pm 1.2$ & $42.0 \pm 1.6$ & $30.0 \pm 0.0$ & $40.9 \pm 6.3$ & $66.2 \pm 0.3$ & --   & --       \\
                               &                               & Avg       & $86.2 \pm 0.1$ & $91.1 \pm 0.2$ & $91.2 \pm 0.3$ & $83.8 \pm 0.2$ & $71.0 \pm 0.0$ & $80.6 \pm 0.1$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Adapter}      & WG        & $77.0 \pm 2.7$ & $87.4 \pm 1.8$ & $76.0 \pm 2.8$ & $69.3 \pm 2.5$ & $67.6 \pm 2.1$ & $76.1 \pm 0.6$ & --   & --       \\
                               &                               & Avg       & $85.3 \pm 0.5$ & $91.9 \pm 0.2$ & $95.0 \pm 0.0$ & $92.7 \pm 0.1$ & $83.1 \pm 1.0$ & $86.4 \pm 0.2$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Group Prompt} & WG        & --             & --             & --             & --             & --             & --             & --   & --       \\
                               &                               & Avg       & --             & --             & --             & --             & --             & --             & --   & --       \\ \midrule
\multirow{6}{*}{CLIP ViT-B/32} & \multirow{2}{*}{Linear Probe} & WG        & $78.3 \pm 0.0$ & $87.6 \pm 0.5$ & $70.7 \pm 0.9$ & $68.7 \pm 0.9$ & $76.8 \pm 0.9$ & $85.3 \pm 0.3$ & --   & --       \\
                               &                               & Avg       & $85.3 \pm 0.0$ & $91.9 \pm 0.1$ & $94.7 \pm 0.0$ & $91.8 \pm 0.2$ & $88.9 \pm 0.7$ & $91.5 \pm 0.0$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Adapter}      & WG        & $83.3 \pm 1.5$ & $87.4 \pm 0.3$ & $76.7 \pm 4.7$ & $70.0 \pm 0.0$ & $82.7 \pm 1.4$ & $86.5 \pm 0.8$ & --   & --       \\
                               &                               & Avg       & $88.9 \pm 0.4$ & $92.0 \pm 0.2$ & $95.1 \pm 0.1$ & $92.3 \pm 0.3$ & $90.7 \pm 0.5$ & $92.1 \pm 0.2$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Group Prompt} & WG        & --             & --             & --             & --             & --             & --             & --   & --       \\
                               &                               & Avg       & --             & --             & --             & --             & --             & --             & --   & --       \\ \midrule
\multirow{6}{*}{CLIP ViT-L/14} & \multirow{2}{*}{Linear Probe} & WG        & $87.9 \pm 0.4$ & $86.3 \pm 0.3$ & $84.0 \pm 0.0$ & $71.3 \pm 3.4$ & $92.5 \pm 0.6$ & $91.7 \pm 0.3$ & --   & --       \\
                               &                               & Avg       & $93.9 \pm 0.2$ & $91.8 \pm 0.1$ & $98.5 \pm 0.0$ & $95.9 \pm 0.1$ & $96.0 \pm 0.4$ & $95.9 \pm 0.2$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Adapter}      & WG        & $88.9 \pm 1.0$ & $88.5 \pm 1.8$ & $86.0 \pm 1.6$ & $77.3 \pm 2.5$ & $90.8 \pm 1.6$ & $92.0 \pm 0.4$ & --   & --       \\
                               &                               & Avg       & $92.4 \pm 0.6$ & $91.6 \pm 0.2$ & $98.4 \pm 0.0$ & $95.9 \pm 0.2$ & $95.2 \pm 0.5$ & $96.3 \pm 0.1$ & --   & --       \\ \cmidrule(l){2-11} 
                               & \multirow{2}{*}{Group Prompt} & WG        & --             & --             & --             & --             & --             & --             & --   & --       \\
                               &                               & Avg       & --             & --             & --             & --             & --             & --             & --   & --       \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\subsection{Improving robustness without group information}
In the prior section, we explored a fundamental question. However, these assumptions may be overly strict. We may not always have group information  

However, if we do not have this group information, then \textfillin{}.

% Poor group-robustness results then from the weight matrix and samples not interacting properly. 

% The above strategies then reflect alternative ways to tease the possible group information out. 

% However, if the original sample embeddings do contain relevant group information, then by either updating the weights of the linear classifier (via (1) linear probes, or us


% The aforementioned strategies can then be thought of as either changing the weight matrix 



% note that zero-shot classification 

% If the input embeddings contain relevant information, then either updating the weights of this linear classification (either via fitting linear probes, or using class embeddings computed from prompts that reflect group information), or transforming the inputs (via adapters) should result in more group-robust classification.

% linear classification via linear probes or class embeddings with prompts that reflect group information. should help. 

% To test this hypothesis


% On the other hand, it is also possible that the zero-shot classification, which is just a log-linear model where the prompt embeddings together make up the weight matrix, does not activate the weights correctly. 

% We then consider training a 

% \header{Group imbalanced / group unknown setting}.



% This suggests 


% it is even possible to improve group robustness using just the precomputed FM embeddings. After all, these same embeddings achieve poor worst-group accuracy when used in zero-shot classification. We consider two competing hypotheses:
% % \begin{enumerate}[leftmargin=*]
%     % \item During pretraining, foundation models learn embeddings that do not contain sufficient information to classify certain groups.
% %     \item The foundation model embeddings actually do retain relevant information needed to properly classify all groups. We just require methods to properly extract this information.
% % \end{enumerate}
% (i) During pretraining, foundation models learn embeddings that do not contain sufficient information to classify certain groups. (ii) The foundation model embeddings actually do retain relevant information needed to properly classify all groups. We just require methods to properly extract this information.

% To validate (i) or (ii), as a first step to improving robustness we train either a linear probe or adapter on top of the foundation model image embeddings with ERM.  If we can significantly improve worst-group accuracy and close the worst-group vs average accuracy gap, then this suggests that the embeddings do retain the relevant group information. 

% \mz{describe the linear probe and adapter method}

% \mz{Describe the training data setup}

% \mz{Include the result table of ERM - will probably need to pick which foundation models and/or datasets to report}

% These results suggest the following properties: 
% \begin{itemize}[leftmargin=*]
%     \item Despite foundation model embeddings resulting in poor group robustness when used in zero-shot classification, the information to classify all groups is present in the embeddings. It just becomes a matter of transforming these embeddings to extract the relevant information.
%     \item If the training data is group-balanced, then training either an adapter or a linear probe on top of these embeddings with ERM is sufficient to significantly improve worst-group accuracy. 
%     \item If the training data is group-imbalanced however, then similar to prior work, training with ERM can actually aggravate the group robustness problem. We then wish to figure out how to extract the relevant information with the available training data without learning training data biases.
% \end{itemize}

% \mz{aside for now - - note that the zero-shot classification paradigm is just a linear classifier $Ax$, where $A$ is the matrix of class or prompt embeddings and $x$ is a sample input vector. Training a linear probe is equivalent to keeping $x$ fixed while updating $A$, while training an adapter is equivalent to keeping $A$ fixed while updating each $x$. }

% Linear probe is training $w^T x$, which can be thought of as fixing the sample embeddings and training and alternate set of prompt embeddings. 

% Adapter is training $z^T f_\theta(x)$, which can be thought of as fixing the class embeddings, and training and alternate set of sample embeddings.


% Breaking this down further, we consider two hypotheses: (i) foundation models learn 

% We consider two hypotheses: (i) during pretraining, foundation models learn embeddings that 





